Improving Experience Replay through Modeling of Similar Transitions' Sets

In this work, we propose and evaluate a new reinforcement learning method, COMPact Experience Replay (COMPER), which uses temporal difference learning with predicted target values based on recurrence over sets of similar transitions, and a new approach for experience replay based on two transitions memories. Our objective is to reduce the required number of experiences to agent training regarding the total accumulated rewarding in the long run. Its relevance to reinforcement learning is related to the small number of observations that it needs to achieve results similar to that obtained by relevant methods in the literature, that generally demand millions of video frames to train an agent on the Atari 2600 games. We report detailed results from five training trials of COMPER for just 100,000 frames and about 25,000 iterations with a small experiences memory on eight challenging games of Arcade Learning Environment (ALE). We also present results for a DQN agent with the same experimental protocol on the same games set as the baseline. To verify the performance of COMPER on approximating a good policy from a smaller number of observations, we also compare its results with that obtained from millions of frames presented on the benchmark of ALE.

==> research_problem.tex <==
\section{Research problem}\label{sec:research_problem}

Once an agent with reinforcement learning has performed a sequence of actions and received a final reward value, knowing how to assign credit or discredit to each state-action pair, to adjust their decision making and improve their effectiveness, consists of a difficult problem, called \textit{temporal credit assignment problem}~\citep{Lin1992}. As this problem is directly related to the effectiveness of the agent, more efficient methods for its approach can also lead to a reduction in the convergence time in their training, which is a critical factor for the application of reinforcement learning to problems each time more complex.

In this sense, Temporal Difference (TD) Learning is one of the main approaches to deal with the problem of credit attribution, but it represents a slow process, especially when the credits have to be propagated by a long sequence of actions. As a consequence, AHC and Q-learning, which represent the first TD-based methods to address reinforcement learning problems, are characterized by high convergence times. To address this problem,~\citet{Lin1992} proposed and analyzed Experience Replay in detail, demonstrating that this is an effective method to accelerate the credit attribution process and, consequently, the convergence time. One of the main motivations for the Experience Replay proposal is the fact that the traditional algorithms, based on AHC and Q-learning, become inefficient when the experiences obtained by trial and error are used only once to adjust the models and then discarded. For ~\citet{Lin1992}, this is a waste, as some experiences can be rare, while others can be expensive to obtain, as in the case of those involving penalties.

Experience Replay has some limitations, being more efficient in the credit propagation if a sequence of experiences is repeated in an order that is temporally opposite to the one in which they were experienced. Also, this process can be more efficient if the $DT(\lambda)$ methods are used with $\lambda>0$, where $\lambda$ is the number of steps used in the calculation. In this way, the temporal difference error used to adjust the models is determined by the discrepancy between multiple consecutive predictions and not just two~\citep{Lin1992}. Another important issue is related to the fact that Experience Replay repeats experiences by sampling. If these experiences defined policies that are very different from what is being learned, selecting a bad action from them, for a same state for which the current policy tends to select a good action, can cause the evaluation and utility functions to be underestimated to this state, if this same action is repeated any number of times.

For Experience Replay to be useful, the agent must repeat only experiences involving actions that will continue to follow the policy that is being learned by the agent. This occurs both for methods based on AHC and Q-learning. In the case of Q-learning, this problem affects methods that use models approximated by neural networks, because whenever the weights of the network that approximates the utility function are adjusted, by backpropagation, for a given state, this affects the network concerning many or perhaps all other states. Thus, if this network is trained from bad experiences many times in a row, the network will tend to underestimate the real usefulness of action-state pairs. However, to prevent overfitting, the agent needs to implement a good strategy to determine if experiences should be remembered and how often they will be repeated~\citep{Lin1992}.

Experience Replay has been used in different approaches present in the literature and discussions about the process of using memories to repeat experiences have relevance and implications in all of them \citep{DBLP:journals/corr/MnihKSGAWR13,mnih2015humanlevel,DBLP:journals/corr/HasseltGS15,DBLP:journals/corr/SchaulQAS15,Wang:2016:DNA:3045390.3045601}. Among the issues commonly pointed out is the need to better explore the repetition of experiences to obtain more significant events during the sampling. There is also a concern that agents with online reinforcement learning update their parameters based on a sequence of experiences and, in their most simplistic form, discard those experiences right after. These updates being strongly correlated makes this approach go against the assumption that the variables are independent and identically distributed, adopted by most algorithms based on stochastic gradients and, therefore, there is no possibility to take advantage of rare experiences that could be useful in the future. For \citet{DBLP:journals/corr/SchaulQAS15}, Experience Replay addresses these issues, because with the experiences stored in memory it is possible to break the correlation between subsequent experiences, interleaving those that are more and less recent to be used in updating the models, while making it possible that rare experiences can be used in the future. Another problem is the fact that the experiences are sampled within a sliding window over the memory. That is, a fraction of these experiences is never repeated before being discarded from memory and another fraction is repeated for the first time only long after being stored.

Experience Replay is a method of fundamental importance for several reinforcement learning algorithms, but it still presents many questions that have not yet been exhausted and problems that are still open. Therefore, this work aims to investigate some of these problems, mainly those related to memory and the use of experiences that can contribute more to the agent's learning, accelerating his learning process.


\subsection{Questions and Hypotheses}\label{sec:questions_hipotheses}

Given the discussions presented in Section~\ref{sec:research_problem}, we can formulate three important questions and raise some theoretical hypotheses:

\textbf{Question 1} - The process of training an agent with learning by temporal difference may lead to the repetition of state transitions with different values of estimates for the action-value function. In this way, it would be possible to define sets of similar transitions, based on the state, action, and immediate reward components of their tuples, and establish some relationship between the transitions of a given set, so that this relationship can be used to evaluate this set as a whole and produce a single transition that represents all the transitions that it contains?

\textbf{Question 2} - It would be possible to obtain a smaller set of transitions than the set of all the transitions already carried out by an agent up to a given moment, but capable of representing all of them, so that this set is more effective for a step of updating of the models which approximate the action-value functions and are adjusted based on the time difference error?

\textbf{Question 3} - Could the use of a smaller set of transitions, but capable of representing the set of all the transitions carried out, contribute to reducing the convergence time of reinforcement learning methods that use temporal difference, thus reducing the time needed for learning?

\textbf{Hypothesis 1} - Consider that a transition is represented as a tuple \((s\textsubscript {t-1}, a\textsubscript{t-1}, r\textsubscript{t}, s\textsubscript{t})\), in which \textit{s\textsubscript{t-1}} and \textit{a\textsubscript {t-1}} refer to the state observed in the previous iteration and the action selected for that state; \textit{r\textsubscript {t}} refers to the immediate return value obtained, once the transition has been made taking the selected action from that state; and \textit{s\textsubscript {t}} refers to the state resulting from the transition.While the agent seeks to learn the best policy, adjusting its value function based on the temporal difference error obtained between the subsequent estimates of the expected discounted total return, state-action pairs leading to the same resulting state can be evaluated more than one time, composing tuples of transitions for which the elements \textit{s\textsubscript{t-1}}, \textit{a\textsubscript{t-1}}, \textit{r\textsubscript{t}}, \textit{s\textsubscript{t}} will be the same, while the results of the \textit{Q\textsubscript{t}} value function are likely will be different, especially if considered as a pair \((r\textsubscript{t}, Q\textsubscript{t})\). Thus, we can consider as similar transitions those in which the elements of states, action, and immediate reward are equal, with a difference only in the values of \textit{Q}, which then becomes a variable related to the tuple of a transition. From this definition, it is possible to form sets of similar transitions based on the state and action components that make up their tuples. If successive transitions associated with the respective values of \textit{Q\textsubscript{t}} are inserted in sets of similar transitions, each time and in the order in which they are carried out during the subsequent iterations throughout the learning, a temporal ordering of these transitions is imposed to each set. If there is a temporal order of these transitions, this implies that there is a temporal order of the values of each element of its tuples, as well as of the values of \textit{Q\textsubscript{t}} associated with them. Thus, we can consider that the values of the elements \textit{s\textsubscript{t-1}}, \textit {a\textsubscript {t-1}}, \textit {r\textsubscript {t}} and \textit {s\textsubscript {t}} remain the same, passing from a similar transition to another, in the order of insertion in a given set. However, we can also consider that the values of \textit{Q\textsubscript {t}} are variable. Therefore, there is a temporal order of variable values for these elements of the transition tuples. If there is a temporal order of variable values in tuples in which there are non-variable elements, they can be represented by anyone of them, obtained from any tuples. In turn, the variable values can be analyzed as a time series to produce a resulting value, for each variable, which allows predicting what their values will be in the next iterations. Thus, it is possible to generate a single transition that represents all transitions in each set of similar transitions, whose tuple is composed of the elements \((s\textsubscript{t-1}, a\textsubscript{t-1}, r\textsubscript{t}, s\textsubscript{t})\), associated with a value \textit{Q'\textsubscript{t}}, where the elements of states, action and immediate reward contain the same values as all similar transitions in the set, but the \textit{Q '\textsubscript{t}} element contains the prediction of the expected Q-value, for those similar transitions contained in the set, in the next iteration that may occur.

\textbf{Hypothesis 2} - Consider that there are sets of transitions grouped as similar transitions based on the elements of states, action, and immediate reward of the tuples that represent them, which are the same for all of them, and that the Q-values associated with these transitions are variable and that these sets are contained in the set of all the transitions already made. If there is a single transition, obtained from each set of similar transitions, so that its elements of states, action, and immediate reward are the same as those of the transitions of its origin set and the associated Q-value is a prediction, made based on the analysis of the values of all transitions in the set, so a new set, formed by these unique transitions, will be smaller than the set of all transitions and, at the same time, will be able to represent it, as it will contain representations of all states, actions and immediate rewards already observed, present in the tuples of the transitions, as well as a representation of all the values of Q-values obtained, represented by the values predicted for \(Q'\textsubscript{t}\) associated with each of them, as these values were obtained from the analysis of each set of similar transitions that originated each of this unique transitions that represent them. When sampling transitions on this smaller set, composed of the unique transitions representing their sets of similar transitions, the chances of a rare transition to be observed are increased, in comparison with a sampling performed on the entire set of performed transitions. Still in this sense, the predicted values \textit{Q'} bring information about how much the transitions on each state-action pair have produced or not good results over the history of similar transitions made. Due to these factors, it is possible that sampling on this smaller set makes the calculation of updating the value function more effective than sampling performed on the set of all transitions.

\textbf{Hypothesis 3} - Repeating transitions previously performed by the agent is considered to be an effective method for reducing the convergence time, but if a sample contains transitions that define policies that are very different from the policy being learned, the selection of a bad action can cause the algorithm underestimates the value function. It is also considered that sampling over a large set of previously stored transitions, using a sliding time window and according to some probability or weight distribution, can still leave out transitions that are rare or expensive to obtain but highly informative. Given these factors, sampling over a smaller set increases the chances of selecting rare and very informative transitions more often, which can contribute to reducing the convergence time in reinforcement learning methods with temporal difference, consequently reducing the training time required for learning.
